Predictive and adaptive maps for long-term visual navigation in changing environments

In this paper, we compare different map management techniques for long-term visual navigation in changing environments. In this scenario, the navigation system needs to continuously update and refine its feature map in order to adapt to the environment appearance change. To achieve reliable long-term navigation, the map management techniques have to (i) select features useful for the current navigation task, (ii) remove features that are obsolete, (iii) and add new features from the current camera view to the map. We propose several map management strategies and evaluate their performance with regard to the robot localisation accuracy in long-term teach-and-repeat navigation. Our experiments, performed over three months, indicate that strategies which model cyclic changes of the environment appearance and predict which features are going to be visible at a particular time and location, outperform strategies which do not explicitly model the temporal evolution of the changes.

==> src/rela.tex <==
%Although probabilistic mapping methods can deal with conflicting measurements, their approach is rooted in the idea that these variations are caused by inherent sensor noise rather than by structural environment change. 
%Thus, these conflicting measurements are generally treated as outliers caused by unwanted noise. 
%Recently, some authors exploited these conflicting measurements in order to obtain information about the world dynamics and proposed representations that model the environment dynamics explicitly.
%These dynamic representations have shown their potential by improving mobile robot localization in changing environments~\cite{churchill,fremen_iros,markov,prediction}. 


The precision and reliability of the self-localisation is largely determined by the accuracy and consistency of the map build by the robot.
One of the main problems of the 
In the context of visual navigation, a robot must ensure that the images have sufficient contrast to identify an adequate number of environmental features necessary for position estimation of the robot relative to its goal.
This not only means that the robot has to adapt the camera settings and feature extraction parameters properly, but also to carefully choose which of the obtained features qualify to store for later use and when to retrieve or discard them from its memory.
In other words, the robot not only needs to make sure that it perceives information relevant to its environment model but also that it can update the environment model based on the perceived information.  
The ability to adapt the settings of the robot perception subsystems, as well as its knowledge bases, is especially crucial in environments which exhibit appearance and structural changes.
The causes for these changes include short-term factors like varying illumination and unpredictable weather and long-term, partially predictable seasonal processes.



One of the first visual SLAM systems, Monoslam~\cite{monoslam}, processes an image stream from an unconstrained-motion monocular camera in real-time, obtaining the trajectory of the camera and a 3D map of salient visual features~\cite{monoslam}.
Another method, the ORB-SLAM~\cite{orbslam,mur2017orb}, allows exploiting stereo and depth information to build both sparse and dense maps of the environment while estimating the camera motion in 6D.
Unlike the aforementioned systems, LSD-SLAM~\cite{lsdslam} and DSO~\cite{dso} do not rely on image feature extraction but create dense, large-scale maps by directly processing the intensities of the image pixels.
A recent, comprehensive review of SLAM systems is presented in~\cite{Cadena16tro-SLAMfuture}.
While being an important component of many navigation systems, SLAM by itself does not control the mobile robot motion, and thus it does not navigate robots per se.
Rather than that, it provides an environment map and a robot position estimate to the motion planning modules, which then guide the robot towards the desired goal.

Thus, one of the typical use of SLAM methods in practice is `teach-and-repeat', where a robot uses SLAM during a teleoperated drive, creating a map of the environment and use this map later on to repeat the taught path~\cite{stereo,teachrepeat,jakobysurfnav}.
This technique is analogous to a popular practice in industrial robotics, where an operator teaches a robot to perform some task simply by guiding its arm along the desired path.
The systems that use SLAM methods within the teach-and-repeat paradigm were extended by techniques like experience-based localisation~\cite{churchill}, feature selection~\cite{Dayoub11} or intrinsic image~\cite{finlaysonOntheremoval}, enabling their long-term deployment in environments that are challenging due to appearance changes~\cite{paton2016bridging,paton2015s,7989238} or difficult illumination conditions~\cite{paton2016dead}.

In the long-term deployments, it's assumed that the robots start and end their forays at their recharging stations with a known position, and occasional loss of localisation is solved by request for human intervention~\cite{strands}. 
Thus, teach-and-repeat methods employed in long-term scenarios do not typically address the kidnapped robot problem. 

Some of the teach-and-repeat systems do not rely on SLAM-built 3D maps of the environment, and employ visual servoing principles while respecting robot dynamics~\cite{kodit}.
For example~\cite{blanc2005indoor,matsumoto} create a visual path, which is a set of images along the human-guided route, and then employ visual servoing to guide robots across the locations these images were captured at.
Similarly,~\cite{segvic} represents the path as consecutive nodes, each containing a set of salient visual features, and uses local feature tracking to determine the robot steering to guide it to the next node.
The authors of~\cite{qualitative} extract salient features from the video feed on-the-fly and associate these with different segments of the teleoperated path.
When navigating a given segment, their robot moves forward and steers left or right based on the positions of the currently recognised and already mapped features.
The segment end is detected by means of comparing the mapped segment's last image with the current view.
The same navigation principle was recently deployed on micro aerial vehicles in~\cite{uav1}. 

At the time when the original SLAM-based teach-and-repeat framework was published~\cite{teachrepeat}, another article~\cite{jfr10} mathematically proved that (while being useful) explicit localisation is not necessary for teach-and-repeat scenarios.
The results of~\cite{jfr10} indicate that to repeat a taught path, camera input needs to be used only to correct the robot heading, leaving the position estimation to odometry.
The mathematical proof showed that for polygonal paths the heading corrections suppress odometric errors, preventing the overall position error of the robot to diverge.
The proof was supported by several long-term experiments~\cite{jfr10,pedre}, where a robot repeatedly traversed long paths in natural environments over the period of one year.
Thus, this SLAMless method showed good robustness to environment changes even without using experience-based or feature-preselection techniques~\cite{pedre}. 
However, the mathematical proof in~\cite{jfr10} was limited to paths consisting of straight segments.
Thus, the system based on~\cite{jfr10} could be taught only polygonal paths in a turn-move manner, and even a slight change of the movement direction during the teaching phase required to stop and turn the robot, which made the teaching tedious and deployment of the system rather impractical.

In this paper, we reformulate the problem presented in~\cite{jfr10} in a continuous rather than a discrete domain.
This allows us to simplify and extend the mathematical proof of~\cite{jfr10} to any continuous trajectory, not only polygonal paths as in~\cite{jfr10}.
A navigation system based on this extended formulation can thus be taught smooth, curved paths, which makes its teaching faster and navigation more efficient. 
 


==> src/vision-loop.tex <==
\subsection{Vision in-the-loop navigation}\label{sec:evaluation0}

The first experiment was used to compare the accuracy of the robot navigation when using the \textit{latest}, \textit{static} and \textit{adaptive} (score-based) map.
Furthermore, we needed to verify if the \textit{adaptive} map performance is sufficient to build datasets for further evaluation.
To do so, we setup a single camera-based localisation system, which was tracking the robot's position with centimetre accuracy~\cite{whycon} during the entire experiment.
Then, we taught the robot a closed path by means of teleoperation during a late afternoon.
This path was only 20m long as we needed to keep the robot within the area covered by the external localisation system.

Since the visual information is used to guide the robot, it is not possible to test more methods at the same time.
Rather, the methods have to be run at a different time, which implies that they are tested in different conditions.
We hypothesise that the \textit{latest} map update causes the robot to drift away from its trajectory even in good conditions, the \textit{static} map strategy is robust to mislocalisation, but it will fail in case of a significant appearance changes in illumination, and the \textit{adaptive} strategy is able to deal with the illumination changes. 
Thus, we taught the robot a path late afternoon and run the three methods in a sequence, so that the \textit{latest} method was tested in normal conditions, the \textit{static} started with a large mislocalisation, and \textit{adaptive} map had to face significant appearance change caused by sunset. 

\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.95\columnwidth]{fig/navigation}
\caption{Robot position error after each autonomous path traversal\label{fig:navigation}}
\end{center}
\end{figure}

After teaching the robot the intended path, we let the robot traverse the taught path autonomously and each time the robot completed the path, we record its position relatively to the taught path start, see Figure~\ref{fig:navigation}.
For the first 8 traversals, we used the \textit{latest map} update scheme.
During the 6th traversal, a minor localisation failure occurred on one of the local maps, corrupting the map and causing gradual divergence of the robot from the path taught.
Thus, at the 8th map repeat, we switched the map update scheme to the \textit{static map} (i.e. the map created during the teaching phase) and the robot gradually corrected its position error.
As it was getting darker, the static map started to fail occasionally due to feature deficiency and thus we switched to the \textit{adaptive map} (with $n$ equal to 50, i.e. exchanging about 10\% of features every time).
Using this map update scheme, the robot continued to traverse the path during and after sunset.
After 35 path traversals, we switched on robot's 4000lm searchlight, and the robot continued to repeat the path.
However, the camera of the external localisation system was saturated with the robot's searchlight, the external localisation system could not track the robot any more.
Thus we measured the position error by measuring the distance of the robot's left rear wheel relatively to its position at the end of the teaching phase. 
Despite of the significant change in the environment appearance, the robot was able to continue to navigate autonomously with position errors around 0.05~m, see Figure~\ref{fig:whycon}.
A video from the experiment performed is provided at~\cite{video}.
This experiment demonstrated that while the \textit{static map} can't handle appearance changes and the \textit{latest map} is prone to occasional localisation glitches.
Since the \textit{score-based map} adaptation proved its ability to guide the robot reliably, we used it for further data gathering. 
%
\begin{figure}[!ht]
\begin{center}
\includegraphics[width=0.95\columnwidth]{fig/whycon}
\caption{Track of the robot position during the first experiment. Taught map is in green and autonomous runs are in red. See a video at~\cite{video}\label{fig:whycon}}
\end{center}
\end{figure}

While the experiment demonstrated that unlike the \textit{static} and \textit{latest} maps, the \textit{adaptive} map can guide the robot in long-term despite the environment changes, it could not be used for a rigorous comparison of more advanced map update strategies.
The problem is that since the navigation method tested is used to guide the robot, it is not possible to test more of the methods at the same time.
For a more thorough comparison, one has to simulate a given map update scheme on datasets gathered by a real robot.

\subsection{Dataset-based evaluation}\label{sec:evaluation1}



